Frame Representation Hypothesis: Multi-Token LLM Interpretability and Concept-Guided Text Generation

Interpretability is a key challenge in fostering trust for Large Language Models (LLMs), which stems from the complexity of extracting reasoning from model's parameters. We present the Frame Representation Hypothesis, a theoretically robust framework grounded in the Linear Representation Hypothesis (LRH) to interpret and control LLMs by modeling multi-token words. Prior research explored LRH to connect LLM representations with linguistic concepts, but was limited to single token analysis. As most words are composed of several tokens, we extend LRH to multi-token words, thereby enabling usage on any textual data with thousands of concepts. To this end, we propose words can be interpreted as frames, ordered sequences of vectors that better capture token-word relationships. Then, concepts can be represented as the average of word frames sharing a common concept. We showcase these tools through Top-k Concept-Guided Decoding, which can intuitively steer text generation using concepts of choice. We verify said ideas on Llama 3.1, Gemma 2, and Phi 3 families, demonstrating gender and language biases, exposing harmful content, but also potential to remediate them, leading to safer and more transparent LLMs. Code is available at https://github.com/phvv-me/frame-representation-hypothesis.git

==> helpers/algorithm.tex <==
\usepackage{algorithm}
\usepackage{algpseudocode}

==> helpers/bibliography.tex <==
\def \bibfile {zotero.bib}

\usepackage[
backend=biber,
style=numeric,
sorting=ynt,
hyperref=auto,
backref=true,
backrefstyle=three,
]{biblatex}

\addbibresource{\bibfile}



==> helpers/code.tex <==
\usepackage[final]{listings}

==> helpers/headers.tex <==
\usepackage{fancyhdr}

\let\Sectionmark\sectionmark
\def\sectionmark#1{\def\Sectionname{#1}\Sectionmark{#1}}

\let\Subsectionmark\subsectionmark
\def\subsectionmark#1{\def\Subsectionname{#1}\Subsectionmark{#1}}

\pagestyle{fancy}
\fancyhf{}
\fancyhead[LE]{\thepage}
\fancyhead[RE]{\Sectionname}
\fancyhead[LO]{\MakeUppercase{\Subsectionname}}
\fancyhead[RO]{\thepage}
\renewcommand{\headrulewidth}{0pt}

==> helpers/numbering.tex <==
\usepackage{titlesec}

% FORMATTING
% Remove section numbers
\makeatletter
\renewcommand{\@seccntformat}[1]{}
\makeatother
% Indent text within section
% \leftskip=2em
% Center section headings
\titleformat{\section}[block]{\Large\bfseries\filcenter}{}{1em}{}
% `enumerate` environment uses (\alph) format
\setlist[enumerate]{label=(\alph*)}

\newcommand{\shrule}{\\ \centerline{\rule{13cm}{0.4pt}}}

==> sections/appendices/liegroupgeo.tex <==
\section{Lie Group Geometry}

A $\numbers$-frame is a set of $\numbers$ linearly independent $\dimension$-dimensional vectors from euclidean space $\vectorspace$, which is represented by a matrix from $\matrixspace$. The Stiefel manifold $\stiefelmanifold{}$ is the set of all orthonormal $\numbers$-frames in $\dimension$-dimensional euclidean vector space $\vectorspace$~\cite[p.~4]{edelman1998geometry}

    \begin{equation}
        \stiefelmanifold{} \coloneqq \set{\mat{F} \in \matrixspace \mid \mat{F}^\top \mat{F} = \mat{I}_\numbers}
    \end{equation}

Furthermore, a $\numbers$-frame can represent more than a fixed set of vectors, but a subspace basis $\subspacemat{F} = \Span(\mat{F}) \subset \vectorspace$. Analogously, the Grassmann manifold $\Grassmann(\numbers, \dimension)$ is the set of all $\numbers$-dimensional subspaces of $\dimension$-dimensional euclidean vector space $\vectorspace$~\cite[p.~4]{Bendokat_2024}

    \begin{equation}
        \Grassmann(\numbers, \dimension) \coloneqq \set{\mat{F}\mat{F}^\top \in \squarematrixspace \mid \mat{F} \in \stiefelmanifold{}}
    \end{equation}

Particularly, these can be taken as manifolds because they can be represented as Lie groups. The subset of all invertible matrices from $\squarematrixspace$ makes the General Linear Group $\GL(\dimension) \coloneqq \set{\mat{A} \in \squarematrixspace \mid \det(\mat{A}) \neq 0}$, and its subset of orthogonal matrices is called the Orthogonal Group $\Or(\dimension) = \set{\mat{Q} \in \GL(\dimension) \mid \mat{Q}^\top \mat{Q} = \mat{I}_\dimension}$. An orthonormal $\numbers$-frame can be made by taking only the first $\numbers$ columns of an orthogonal matrix, so the space of all orthonormal frames becomes the quotient space $\stiefelmanifold{} \simeq \orthogonalframegroup$. Analogously, the space of all $\numbers$-dimensional subspaces becomes the quotient space $\Grassmann(\numbers, \dimension) \simeq \subspacegroup$. Whereas these are considered two distinct objects, frames and subspaces can be unified by introducing the concept of flags.~\cite{edelman1998geometry,Bendokat_2024}

\begin{definition}[Flag]
    A flag $\flag{F} = \{ \subspace{F}_i \}_{i = 1}^{\flagtypesize}$ is a nested sequence of subspaces 
    
    \begin{equation}
        \varnothing \subset \subspace{F}_1 \subset \subspace{F}_2 \subset \dots \subset \subspace{F}_\flagtypesize \subset \vectorspace
    \end{equation}
\end{definition}

In matrix space, $\flagmat{F}_{(\flagtype)}$ represents a flag of type $\flagtype$, $0 < \numbers_1 < \numbers_2 < \dots < \numbers_\flagtypesize < \dimension$, built from sub-frames within an orthonormal $\numbers_\flagtypesize$-frame $\mat{F}$
\begin{equation}
    [\mat{F}_{\dots \numbers_1}] \subset [\mat{F}_{\dots \numbers_2}] \subset \dots \subset [\mat{F}_{\dots \numbers_\flagtypesize}] = \subspacemat{F} \subset \vectorspace
\end{equation}
where $\mat{F}_{\dots \numbers_i}$ is the sub-frame containing the first $\numbers_i$ vectors of $\mat{F}$. We denote complete flags over $\mat{F}$ simply as $\flagmat{F}$, \ie, $\flagmat{F}_{(\completeflagtype)} = \flagmat{F}$

The set of all flags of type $(\flagtype)$ constitutes the Flag manifold $\genericflagmanifold$, but given flags are sequences of $\flagtypesize$ nested subspaces represented by a single matrix, the flag manifold must be a quotient space with $\flagtypesize + 1$ equivalences classes $$\genericflagmanifold \simeq \flaggroup$$ where $\numbers_0 = 0$ and $\numbers_{\flagtypesize + 1} = \dimension$~\cite{ye2022optimization}

Such a remark implies Flag manifolds generalize both Stiefel and Grassmann manifolds. Indeed, $\completeflagmanifold{} \simeq \orthogonalframegroup \simeq \stiefelmanifold{}$, while $\Flag(\numbers, \dimension) \simeq \subspacegroup \simeq \Grassmann(\numbers, \dimension)$. Therefore, while the subspace representation is invariant to swaps of vectors (rotations), the flag introduces regions of invariance because it is a nested sequence, so some vectors can swap with others but they are not free to swap with any other vector. In turn, this also adds a notion of ordering to the vectors and subspaces, making it equivalent to a frame in the complete case. Notice however, this is an equivalence in how these entities are represented in the orthogonal group, while the underlying geometric object can still be regarded as distinct, \eg, a frame is not necessarily a sequence of orthonormal 1-dimensional subspace, but both are represented by the same matrix.
